Towards QoS-Aware Recommendations

In this paper we propose that recommendation systems (RSs) for multimedia services should be "QoS-aware", i.e., take into account the expected QoS with which a content can be delivered, to increase the user satisfaction. Network-aware recommendations have been very recently proposed as a promising solution to improve network performance. However, the idea of QoS-aware RSs has been studied from the network perspective. Its feasibility and performance performance advantages for the content-provider or user perspective have only been speculated. Hence, in this paper we aim to provide initial answers for the feasibility of the concept of QoS-aware RS, by investigating its impact on real user experience. To this end, we conduct experiments with real users on a testbed, and present initial experimental results. Our analysis demonstrates the potential of the idea: QoS-aware RSs could be beneficial for both the users (better experience) and content providers (higher user engagement). Moreover, based on the collected dataset, we build statistical models to (i) predict the user experience as a function of QoS, relevance of recommendations (QoR) and user interest, and (ii) provide useful insights for the design of QoS-aware RSs. We believe that our study is an important first step towards QoS-aware recommendations, by providing experimental evidence for their feasibility and benefits, and can help open a future research direction.

==> AdditionalPlots.tex <==
\begin{minipage}[t]{0.46\linewidth}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/abandonment.eps}
\label{fig:abandonment}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/cdf_interest.eps}
\label{fig:cdf_interest}
\end{minipage}

\begin{minipage}[t]{0.46\linewidth}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/cdf_intNext_qorPrev.eps}
\label{fig:cdf_intNext_qorPrev}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/chrcrrfixed.eps}
\label{fig:chrcrrfixed}
\end{minipage}

\begin{minipage}[t]{0.46\linewidth}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/chrXindex.eps}
\label{fig:chrXindex}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/chrXqorXint.eps}
\label{fig:chrXqorXint}
\end{minipage}

\begin{minipage}[t]{0.46\linewidth}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/intsoi.eps}
\label{fig:intsoi}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/intsoibuckets.eps}
\label{fig:intsoibuckets}
\end{minipage}

\begin{minipage}[t]{0.46\linewidth}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/qorsoibuckets.eps}
\label{fig:qorsoibuckets}
\includegraphics[width=1\columnwidth]{./figures/figuresSavvas/qorsoifixed.eps}
\label{fig:qorsoifixed}
\end{minipage}

==> Introduction.tex <==
% \subsection{Motivation}
Multimedia delivery services, such as online video (e.g., YouTube, Netflix, Hulu), audio (e.g., Spotify, Deezer), live streaming for gaming (e.g., Twitch.tv), content over social media (e.g., Facebook), etc., use recommendation systems (RSs) to best satisfy the users, and/or maximize their engagement in the service. Recommendations are for contents that are predicted to have high probability to be selected and liked by the user. Predictions are mainly based on user interests, history, content/user similarity scores, etc. Recommendations may also take into account the \textit{context} of a viewing session (e.g., location, time, type of device, user activity, environment)\myblue{~\cite{villegas2018characterizing,agagu2018context, adomavicius2011context, baltrunas2011matrix, nguyen2014gaussian, pagano2016contextual, almutairi2017context, wang2017context}}%~\cite{villegas2018characterizing}
.



However, RSs for multimedia content services are currently agnostic to the \textit{quality of service (QoS)} with which the content is delivered to the user\myblue{, and QoS has not been considered as a dimension of the ``context''}. Yet, everyday experience and numerous studies suggest that QoS has a major effect on the overall user experience (QoE) and engagement in the service~\cite{conviva2015,ericsson2018,krishnan2013video,nam2016qoe}. For instance, the network congestion or topology (e.g., cached content) may affect the bit-rate, the latency, and start-up delay of a video streaming, causing annoying impairments such as re-buffering or changes in bit-rates~\cite{nam2016qoe,doan2019tracing}. Such poor QoS delivery can be detrimental for the user QoE~\cite{conviva2015,ericsson2018}. This concern is expected to be amplified in the future, as video delivery increasingly dominates network traffic, the bar for acceptable video quality is raised, and larger portions of such content must be delivered over mobile networks, which will struggle to serve all content requests in high-QoS~\cite{ericsson2018,cisco2018}. 
%\akis{does any of the above cited works make the case that current QoS is often subpar?? what the above is saying is ``IF QoS is bad, then yeah it affects QoE and should be considered''. But what if I said ``but QoS is excellent these days! so what you propose would be useless most of the time''. Does one of these studies counters this comment? what about the YouTube delay/qos study you showed us?} 


% \subsection{Proposed Idea and Contributions}

In this paper, our major contribution is twofold.

\myitem{QoS-aware recommendations.} We propose to explicitly take QoS (or, the specific network conditions) into account in RSs for video and multimedia content delivery. Recommending content that can be delivered with high QoS (e.g., videos cached close to users) can lead to improved user experience. For example, if two videos have similar predicted interest to a user, but current network conditions suggest that one of them would likely suffer from poor quality streaming, the RS should recommend the high-QoS video. Our claim is that the user will then enjoy the viewing more, and possibly stay longer in the service. 

Some very recent works in the area of communication networks have considered the co-design of recommendation and network optimization algorithms~\cite{sermpezis2018soft,chatzieleftheriou2019jointly,kastanakis2018cabaret,zhu2018coded,lin2018joint,giannakas2018show,song2018making}. Initial results are very promising for the \textit{network performance}: nudging recommendations towards network-friendly content delivery can bring significant improvements to network capacity, congestion, or energy consumption. While these findings reveal a new potential, they have two shortcomings: (i) recommendation quality and user experience was a secondary goal, i.e., considered as ``something not to get too distorted'' while improving network performance; (ii) the impact of this (recommendation) nudging and potential (QoE) distortions is only speculated, but is not validated with real users.  

%\akis{I think this last subsection needs work. the contributions (idea + experiment results + RS design implications) are not clearly stated yet. It's all there in principle, but don't like the marketing yet. also we might want to write 1 contribution with 1 key message, previewing the results essentially}

\myitem{Experimental study: real user trade-offs.} 
Hence, some key questions arise: ``Should one design QoS-aware recommendation algorithms that explicitly target user experience?''. ``How would real users factor in QoS, content interest, and Quality of Recommendations (QoR) into their overall experience?" While the earlier toy example, with two equally interesting contents, is straightforward, less obvious tradeoffs arise in practice. For example, how should a recommender choose between a content with predicted QoS rating 3, and interest 4, and another with QoS 4 and interest 3? What about $\{4,3\}$ and $\{3,5\}$, respectively? Should a RS favor the content of higher interest to the user or of higher QoS? And does the answer change, depending on the scenario? Unfortunately, we currently lack answers to the above questions. 

This work aims to be the first step towards answering such questions, by evaluating for the first time the joint impact of recommendation algorithms and QoS with experiments with real users. We provide \textit{initial experimental results and insights on the design of QoS-aware RSs}, which we believe can motivate further research and advances in the design of QoS-aware RSs. \myblue{Specifically, our results are the first to provide experimental evidence that:
\begin{itemize}[leftmargin=*]
    \item Carefully nudging recommendations towards network friendly video delivery is not perceived as intrusive by users. This is a positive message for the feasibility of the recently proposed paradigm for joint network and RSs design, which can bring significant improvements in network performance. 
    \item QoS-aware recommendations lead to a higher overall user satisfaction as well, in addition to the network benefits.    
    \item Recommending a high-QoS video is of equal (at least) importance to recommending an interesting (for the user) video, for refraining users from abandoning a session. Hence, by taking QoS into account in recommendations, can lead to higher retention rates and revenues for the content provider.
\end{itemize}
In total, }%
our findings suggest that QoS-aware recommendations can benefit both the users (better experience) and the RS (higher retention rate), adding to the already shown gains for the network. Moreover, we identify complex relationships between the quality of recommendations, the QoS, and the user satisfaction, which indicates that the design of QoS-aware RS is far from trivial and requires further investigation.

The remainder of the paper describes the experiments (Section~\ref{sec:experiments}), provides initial results and insights (Section~\ref{sec:results}), and discusses relevant issues, such as, relation to existing approaches and technical feasibility (Section~\ref{sec:discussion}). We conclude the paper in Section~\ref{sec:conclusion}.

%\akis{A question that easily arises reading the intro is: ``but how can the RS know all this info?'' It is now moved I guess in the discussion section...but maybe we should make a brief mention of this somewhere in the intro. E.g., ``we discuss how such information can be known to the RS at the end of the paper''}


%\pavlos{cite the YouSlow work(s), to say that the concept has wider (than only cellular networks) applicability}


% \myitem{Contributions:}
% \begin{itemize}
%     \item Introduce the idea of QoS-aware design of recommendation systems, aiming to improve user satisfaction and/or retention rate.
%     \item Initial experimental study with real users, collection of data and analysis of their behavior wrt. to the RSs and QoS.
%     \item \pavlos{secondary contribution} We intent to make our code for the platform available to facilitate future experimentation and evaluation of QoS-aware algorithms. 
% \end{itemize}

==> ML_model.tex <==
The analysis of our results, e.g., see Fig.~\ref{fig:qoe-of-int-qos}, indicate that the relation between user \textit{interest}, \textit{QoS}, and \textit{QoE} is highly non-linear. Similar patterns can be observed in  Fig.~\ref{fig:qoe-of-qor-qos} the interplay of \textit{QoR}, \textit{QoS}, and \textit{QoE} as well. Hence, previously proposed simple linear models~\cite{ding2014combining} may not be adequate in practice

Our goal in this section is to (i) better understand how the \textit{interest} (or, recommendations -- \textit{QoR}) and \textit{QoS} jointly affect the experience of a user, and at the same time to (ii) take initial steps towards modeling these joint effects.

\myitem{Overview of modeling approach.} Towards achieving the above goal, we select to model the interplay of \textit{QoS}, \textit{QoR}, and \textit{interest} with generalized linear models (GLM), which allow to capture complex effects and that the same time can be interpretable and reveal insights. \red{This choice is in line with the increasing demand (from the AI community in general~\cite{}, and the RS community in particular~\cite{}) for tractable/explainable ML models and AI algorithms.} Moreover, our choice is also motivated by the fact that the size of our dataset and the experimental setup for its collection, would not be able to support an accurate representation of an operational service (e.g., YouTube). For instance, building and training a deep learning model (neural network) that could fit our data, but could not be interpreted, would be of limited practical value. 

To this end, in the following, we first carefully select the set of features to be used in such a GLM (Section~\ref{sec:feature-selection}), and then design a model to predict QoE and analyze its structure to derive interesting insights (Section~\ref{sec:model-and-insights}).
Our ultimate goal is to achieve a good trade-off between simplicity/explainability and accuracy; our results indicate that we can achieve this.



\subsection{Feature Selection}\label{sec:feature-selection}

\myitem{Basic features.} Our dataset contains the user ratings for \textit{QoS}, \textit{QoR}, and \textit{interest}; this is information can be known or approximated by the content provider. These are the three basic features that can be taken into account to predict the QoE. Let us denote these basic features as $x_{i}$, $i=1,2,3$.

\myitem{Meta-features.} To capture the more complex effects that the basic features have on the QoE (see above analysis and discussion), we can take into account additional ``meta-features'', namely, non-linear functions of single features $g(x_{i})$ (e.g., squares, logarithms) or complex functions of combinations of features $g(x_{i},x_{j})$ (e.g., products, ratios). However, there are unlimited options for possible meta-features, and we need to narrow down the set of the meta-features we consider and select only the most important. 

We start from the single feature functions $g(x_{i})$ and test a wide range of different functions $g$ as predictors of the QoE ratings, i.e., $\hat{QoE}=g(x_{i})$. Our findings show that linear functions ($g(x_{i})=\alpha\cdot x_{i}+\beta$) perform approximate better the QoE. This indicates that \textit{considering non-linear functions of the  features as meta-features would not significantly improve the predictive performance of a model}.\pavlos{is there a more formal way to test/show this?}

We then proceed to combinations of feature pairs, and test different linear and non-linear regression models $\hat{QoE}=g(x_{i},x_{j})$. Table~\ref{tab:ml-model-fit-mae} presents the results for the accuracy of the models we tested: specifically, from our dataset, we first removed the outliers\footnote{Outliers are considered the samples where the maximum rating for QoS, QoR, Int is lower than the QoE rating, or the mimimum rating for QoS, QoR, Int is higher than the QoE rating.}, and then randomly split the dataset into the training set (\red{XX}\% of the total samples) and the test set (\red{XX}\% of the total samples); then, we trained the models over the training set, and derived the mean absolute error (MAE) on the test set\footnote{The MAE is calculated as $MAE = \sum_{s}|\hat{QoE}_s - QoE_{s}|= \sum_{s}|g(x_{i}, x_{j}) - QoE_{s}|$, where $s$ the samples in the test dataset.}. 



\begin{table}[h]
\centering
\caption{Mean absolute error, MAE, of different models (rows) with different features (columns), trained using Cross Validation (k=5). \pavlos{@Savvas: add column for QoR,Int; try Decision Tree Regressor instead of random forest}}
\label{tab:ml-model-fit-mae}
\begin{tabular}{c|l|ccc}
{Type of}& {Model} &  \multicolumn{3}{c}{Features}      \\
{model}  & {(regression)}  &  {QoS, Int} &  {QoS, QoR} & {Int, QoR}\\
\hline
\multirow{3}{*}{linear }
    & {Linear} &  {0.69} &  {0.80}  & {0.87}\\
    & {Logistic}  &  {0.65} &  {0.81}  & {0.89}\\
    & {Ordinal}       &  {0.60} &  {\textbf{0.75}} & {\textbf{0.81}}\\
\hline
\multirow{4}{*}{non-linear}
    & {SVR}       &  {0.60} &  {0.77} & {0.85}\\
    & {Rnd. Forests}    &  {0.58} &  {0.85}  & {0.87}\\
    & {Decision Trees}    &  {0.65} &  {0.82}  & {0.91}\\
%{SVC}       &  {0.57} &  {0.78}  \\
    & {MLP}       &  {\textbf{0.57}} &  {0.78} & {0.90}
\end{tabular}
\end{table}

% Table~\ref{tab:ml-model-fit-mae} present the MAE of different models trained over the entire dataset, from which outliers\footnote{Outliers are considered the samples where the maximum rating for QoS, QoR, Int is lower than the QoE rating, or the mimimum rating for QoS, QoR, Int is higher than the QoE rating.} are previously removed (the relative performance of models is similar to the case of not removing outliers; the absolute MAE decreases, e.g., the best MAE is 0.5 and is achieved by SVR).
% \begin{table}[h]
% \centering
% \caption{Mean absolute error, MAE, of different models (rows) with different features (columns), trained in the entire dataset without outliers; in regression models, the QoE prediction is rounded to the closer integer.}
% \label{tab:ml-model-fit-mae}
% \begin{tabular}{l|cccc}
% {}     &  {QoS, Int} &  {QoS, QoR} &  {QoR, Int} &  {min\{QoS,Int\},} \\
% {}     &  {} &  {} &  {} &  {max\{QoS,Int\}} \\
%  \hline
% {Logistic Regression}  &  {0.66} &  {0.52} &  {0.50} &  {0.53} \\
% {Linear Regression}    &  {0.49} &  {0.52} &  {0.46} &  {0.44} \\
% {LDA}       &  {0.52} &  {0.47} &  {0.46} &  {0.45} \\
% {MLP Regression}       &  {0.46} &  {0.42} &  {0.41} &  {0.49} \\
% {SVR}       &  {0.35} &  {0.37} &  {0.37} &  {0.35} \\
% \end{tabular}
% \end{table}


The results for the pair $\{QoS,Int\}$ show that non-linear models better capture the joint effect of these features (and thus are aligned with our analysis in Section~\ref{}; see Fig.~\ref{}). In particular, among the models we tested, the Multi-layer perceptron (MLP) regression model (in which we used a neural network with two hidden layers with \red{16} nodes each) performs best. 
%In the contrary, linear models (Linear Regression) and models that use linear combinations of the features (Logistic Regression, Ordinal Regression) have higher MAE. 
Since, MLP is not directly interpretable, we use a visualization of its predictions in Fig.~\ref{fig:2D-qos-int-MLPR} to obtain insights about how \textit{QoS} and \textit{Int} jointly affect the QoE. The visualization reveals an interesting pattern: the QoE could be approximated by a function $g(QoS,Int)\approx \min\{QoS, Int\}$ or $g(QoS,Int)\approx QoS \cdot Int$ (apart from the visual inspection, we tested and verified that the behavior of these functions are close to the MLP). In fact using either function (minimum or product) is equivalent; in our dataset the quantities $\min\{QoS, Int\}$ and $QoS \cdot Int$ have a Pearson correlation coefficient equal to 0.98. Hence, in the following we consider only the minimum. %(see Table~\ref{tab:correlation-product-min})

Proceeding in the same way for the other combinations of the basic features, we resulted in similar findings (which we omit due to space limitation); in some cases there exist notable differences in the observed patterns though, e.g., as shown in Table~\ref{tab:ml-model-fit-mae} the joint effect \textit{QoS} and \textit{QoR} is equally well approximated by a linear model, even though its prediction power is much lower (cf. the higher MAE). In total, our analysis indicates that \textit{the functions $g(x_{i},x_{j})=min\{x_{i},x_{j}\}$ (and $g(x_{i},x_{j})=max\{x_{i},x_{j}\}$) are good candidates for meta-features, since they are both reasonable approximations and can be easily interpreted}. In the contrary we did not consider functions of the products of features (which are equivalent to the minimum) and ratios of the features (which were found to not be statistically dependent to the QoE ratings, e.g., the p-value of a chi-square test for $\frac{QoS}{Int}$ is $\sim 0.3$ ).

\myitem{Selected features: $x_{1}=QoS, x_{2}=QoR, x_{3}=Int$, and $min\{x_{i},x_{j}\}$, and $max\{x_{i},x_{j}\}$, $\forall i,j\in\{1,2,3\}$.}




%Figure~\ref{fig:2D-MLPR} visualizes two MLPR models for predicting the QoE from the features QoS and Int (Fig.~\ref{fig:2D-qos-int-MLPR}), and QoS and QoR (Fig.~\ref{fig:2D-qos-qor-MLPR}).




\begin{figure}
\centering
\subfigure[QoS vs. Int]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__QoS_vs_Int__MLPRegressor__rm_outliers_True.eps}\label{fig:2D-qos-int-MLPR}}
\hspace{0.05\linewidth}
\subfigure[QoS vs. QoR]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/featureSelection.eps}\label{fig:MAE-vs-nb-features}}
\caption{(a) QoE predictions of MLP regression model with features QoS and Int. The axes correspond to the feature values (from 1 to 5 stars), the colored areas denote the QoE predictions (from 1 to 5 stars; dark blue corresponds to 1 and light green to 5), and the lines are the boundaries between the different QoE areas. (b) MAE of Ordinal Regression model vs. number of top features (from Table~\ref{table:weights-ordinal}) used.}
\end{figure}

% \begin{figure}
% \centering
% \subfigure[QoS vs. Int]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__QoS_vs_Int__MLPRegressor__rm_outliers_True.eps}\label{fig:2D-qos-int-MLPR}}
% \hspace{0.05\linewidth}
% \subfigure[QoS vs. QoR]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__QoS_vs_QoR__MLPRegressor__rm_outliers_True.eps}\label{fig:2D-qos-qor-MLPR}}
% %\subfigure[min\{QoS,Int\} vs. max\{QoS,Int\}]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__min_QoS_Int_vs_max_QoS_Int__MLPRegressor__rm_outliers_True.eps}\label{fig:2D-qos-int-MLPR}}
% \caption{QoE predictions of MLP regression model with parameters/features (a) QoS and Int, and (b) QoS and QoR%min\{QoS,Int\} and max\{QoS,Int\}
% . The axes correspond to the feature values (from 1 to 5 stars), the colored areas denote the QoE predictions (from 1 to 5 stars; dark blue corresponds to 1 and light green to 5), and the lines are the boundaries between the different QoE areas.}
% \label{fig:2D-MLPR}
% \end{figure}



% Moreover, the two meta-features $QoS\cdot Int$ and $\min\{QoS,Int\}$ are similar; this is indicated by their (Pearson) correlation coefficient value, which is 0.98 (see Table~\ref{tab:correlation-product-min}). Hence, we can use one of them, i.e., either the product or the minimum.
% \begin{table}[h]
% \centering
% \caption{Correlation coefficient between the meta-features $X\cdot Y$ and $\min\{X,Y\}$, where $X,Y\in\{QoS, QoR, Int\}$.}
% \label{tab:correlation-product-min}
% \begin{tabular}{c|c}
% {$X,Y$}   &  Correlation\\
% \hline
% QoS, Int  & {0.98} \\
% QoS, QoR  & {0.97} \\
% QoR, Int  & {0.97}
% \end{tabular}
% \end{table}



\subsection{Model and Insights}\label{sec:model-and-insights}

We proceed to design an interpretable model, namely, a GLM that uses a linear combination of the selected features, i.e., $\hat{QoE} = f(\sum_{i} w_{i}\cdot g_{i})$ where $g_{i}$ denotes a feature (such as QoS or min\{QoS,Int\}), $w_{i}$ is the weight of the feature $g_{i}$% (the larger the absolute value of the weight, the higher the importance of the meta-feature in the model)
, and $f$ the model function (e.g., $f(x)=x$ for Linear Regression, or $f(x)= \frac{1}{1+e^{-x}}$ for Logistic Regression).

While we use a GLM, by including meta-features that are non-linear combinations of the basic features, allows to capture their non-linear effects on QoE (thus advancing from previous simple/linear models~\cite{ding2014combining}).

\myitem{Ordinal Regression (OR) vs. other GLMs.} %
% \myitem{Ordinal Regression (OR) is the best performing GLM by predicting in \red{XX}\% of the cases the QoE within $\pm1$ of the real user rating.} %
We consider three different GLMs, namely, \textit{Linear}, \textit{Logistic}, and \textit{Ordinal} regression\footnote{Ordinal Regression is a model that is applied in cases where the variables take values in an ordered scale (e.g., 1 to 5), and is commonly used for modeling human levels of preference.}, using all the features selected in Section~\ref{sec:feature-selection}. We train the models on \red{XX}\% of the samples in our dataset, and calculate their MAE \red{and prediction accuracy} over the remaining samples; \red{we use 5-cross validation to calculate the average MAE values(???)}. Table~\ref{tab:performance-ordinal} presents the prediction results, which show that Ordinal Regression outperforms other GLMs. In particular, its \textit{QoE} predictions deviate on average from the real ratings by $\pm \red{XX}$; a more detail look shows that \red{XX}\% of the predictions are exact, \red{XX\%} are within $\pm1$ of the real rating, and only \red{XX}\% predictions clearly cannot capture the experience declared by the user.
\begin{table}[h]
\centering
\caption{Performance of models.}
\label{tab:performance-ordinal}
\begin{tabular}{c|c|c|ccc}
{} &Model & MAE & \multicolumn{3}{c}{prediction error, $|\hat{QoE}-QoE|$:}   \\
{}& {} & {} & {$=0$}& {$=1$}& {$>1$}\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{GLMs}} 
    & Ordinal & {0.54} & \red{5X\%} & \red{3X\%} &\red{1X\%}\\
    & Linear & {0.60} & \red{XX\%} & \red{XX\%} &\red{XX\%}\\
    & Logistic & {0.56} & \red{XX\%} & \red{XX\%} &\red{XX\%}\\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{Baselines}} 
    &Dummy & {1.26} & \red{5X\%} & \red{3X\%} &\red{1X\%}\\
    & Vanilla-RS & \red{0.XX} & \red{XX\%} & \red{XX\%} &\red{XX\%}\\
    %& w/o meta-features & \red{0.XX} & \red{XX\%} & \red{XX\%} &\red{XX\%}  \\
    & OR(QoS,QoR,Int) & {0.58} & \red{XX\%} & \red{XX\%} &\red{XX\%}    
\end{tabular}
\end{table}

\myitem{OR vs. baseline recommenders.} To better quantify the added value of the proposed model, we compare it with baseline models, namely: (i) \textit{dummy}: always predict $\hat{QoE}=3$, (ii) \textit{vanilla RS}: a RS that does not take QoS into account and predicts $\hat{QoE}=Int$, (iii) \textit{simple QoS-aware RS}: an Ordinal Regression model that does not uses meta-features, i.e., $\hat{QoE}=OrdinalRegression(QoS,QoR,Int)$. \pavlos{Results show that ... [we perform better: the achieved performance is X times the minimum, it outperforms a QoS-unaware RS (which are used today) by X, and the importance of using meta-features is XX]}

%\footnote{\url{https://scikit-learn.org/stable/modules/model_evaluation.html#dummy-estimators}}

\myitem{Feature importance in prediction accuracy.} The main motivation for using a GLM is interpretability of results. In particular, the weights $w_{i}$ indicate the relevant importance of the feature $g_{i}$, i.e., the larger the absolute value of the weight, the higher the importance of the meta-feature in the model. In this context, we present in Table~\ref{table:weights-ordinal} the weights of all the features in the model, and discuss some key insights stemming from them.

\textit{Observation 1:} The minimum of the user \textit{Int} and \textit{QoS} plays the most significant role. In fact, the weight of this feature is two times higher than the second largest weight. This clearly indicates that \textit{users cannot not be highly satisfied unless \textbf{both} the video is delivered in good quality and lies within their interests}; in other words, recommending a video with poor QoS, is equally bad to a non-relevant recommendation. This finding further supports the motivation of our paper, and stresses the need for QoS-aware RSs in multimedia services.

\textit{Observation 2:} The feature $max\{QoR,Int\}$ appears as the second most important factor. While this term is less straightforward to explain, an interpretation is that \textit{the users can be satisfied either if they are interested \textbf{either} in the video they currently watch (Int) \textbf{or} in the videos they are recommended to watch next (QoR)}. Here it is important to note that \textit{Int} and \textit{QoR} are not highly correlated (Pearson corr. coefficient 0.42).

While the above observations may seem intuitive (in retrospect), our analysis (i) provides experimental evidence to support them, and (ii) is a first step towards quantifying these effects. 

\textit{Observation 3:} \pavlos{This is not anything wow, we could omit it.} The sum of the weights of the features where the QoS appears, gives 0.63; the corresponding values for QoR and Int, are 0.39 and 0.63. This indicates that QoS and Int have an similar contribution in user experience, which is significantly higher than this of QoR. 

% \begin{table}[h]
% \centering
% \caption{Weights of features in Ordinal Regression model}
% \label{table:weights-ordinal}
% \begin{tabular}{l|r}
% {feature $g_{i}$}     & {weight $w_{i}$}\\
% \hline
% $\min\{QoS,Int\}$     & 0.38\\
% $\max\{QoR,Int\}$     & 0.19\\
% $Int$               & 0.15\\
% $QoS$               & 0.15\\
% $\min\{QoS,QoR\}$     & 0.10\\
% %other features      & $<$0.10
% \hline
% $\max\{QoS,QoR\}$     & 0.08\\
% $\max\{QoS,Int\}$     & -0.08\\
% $QoR$               & 0.03\\
% $\min\{QoR,Int\}$     & -0.01
% \end{tabular}
% \end{table}


\begin{table}[h]
\centering
\caption{Weights of features in Ordinal Regression model}
\label{table:weights-ordinal}
\begin{tabular}{l|r||l|r}
{feature $g_{i}$}     & {weight $w_{i}$} & {feature $g_{i}$}     & {weight $w_{i}$}\\
\hline
$\min\{QoS,Int\}$     & 0.38 & $\max\{QoS,QoR\}$     & 0.08\\
$\max\{QoR,Int\}$     & 0.19 & $\max\{QoS,Int\}$     & -0.08\\
$Int$               & 0.15 & $QoR$               & 0.03\\
$QoS$               & 0.15 & $\min\{QoR,Int\}$     & -0.01\\
$\min\{QoS,QoR\}$     & 0.10\\
\end{tabular}
\end{table}

\joao{\myitem{An alternative approach to the modelling.} 
Let us recall that each original feature (QoS, Ind, QoR), and the original response QoE, can take integer values from 1 to 5.
For each one of these three original features, we created a new binary feature which can be “Low”, if the original feature is at most 3; or “High”, if the original feature is at least 4. The same procedure was also applied to the response QoE. Therefore, we got three binary features and a binary response. 
A preliminary statistical analysis of the data, based on building contingency tables and computing the chi-square test statistic for pairwise independence, showed that:
\begin{itemize}
  \item 	Regarding their separate predictive power for QoE, QoS is the strongest feature (Chi-square = 137.77), followed by Interest (Chi-square = 117.22) and QoR (Chi-square = 43.91).
\item	Fortunately, all three features are weakly related to each other: Chi-square(QoS, Int) = 26.55,  Chi-square(QoS, QoR) = 6.22, Chi-square(QoR, Int) = 23.87.
\item	Considering the dependence relationship between a pair of features and QoE, we got: Chi-square[(QoS, Int), QoE] = 223.16, Chi-square[(QoS, QoR), QoE] = 167.01, Chi-square[(QoR, Int), QoE] = 135.57. Then, (QoS, Int) seems to be the most promising pair of features for predicting QoE.
\end{itemize}
Our final goal here was to build a classifier, namely, a rule capable of predicting whether QoE would be High or Low, given:
\begin{itemize}
\item	A combination of the input binary features (e.g., QoS = High, Int = Low, QoR = High);
\item	The overall proportion of High QoE sessions in the target population.
\end{itemize}
Our results are summarized in the following table, where:
\begin{itemize}
\item The three first columns indicate each one of the eight possible input feature combinations.
\item The labels on top of the remaining columns indicate the overall proportion of High QoE sessions, varying from 0.1 to 0.9.
\item The contents of these remaining columns indicate the predicted QoE (Low or High).
\end{itemize}
\begin{center} 
\begin{tabular}{| c | c | c || c | c | c | c | c | }
\hline
 QoS & Int & QoR & 0.1 & 0.2 & 0.3 & 0.4 & 0.5 \\ 
 \hline
 Low & Low & Low & Low & Low & Low & Low & Low \\  
 Low & Low & High & Low & Low & Low & Low & Low \\
 Low & Low & High & Low & Low & Low & Low & Low \\
 Low & High & High & Low & Low & Low & Low & Low \\
 High & Low & Low & Low & Low & Low & Low & Low \\
 High & Low & High & Low & Low & Low & Low & High \\
 High & High & Low & Low & Low & High & High & High \\
 High & High & High & High & High & High & High & High \\   
 \hline
 QoS & Int & QoR & 0.6 & 0.7 & 0.8 & 0.9 & \\
 \hline
 Low & Low & Low & Low & Low & Low & Low & \\  
 Low & Low & High & Low & Low & Low & Low & \\
 Low & Low & High & Low & Low & Low & High & \\
 Low & High & High & High & High & High & High & \\
 High & Low & Low & Low & Low & High & High & \\
 High & Low & High & High & High & High & High & \\
 High & High & Low & High & High & High & High & \\
 High & High & High & High & High & High & High & \\
\hline
\end{tabular}
\end{center}
In order to build this classifier from the available dataset, we used a statistical methodology based on a Naïve Bayes approach. The procedure assumes that the binary features are conditionally independent, given the binary response.
The classifier accuracy was estimated by cross-validation to be 86\%, if the overall proportion of High QoE sessions is around 50\% (the one prevailing in our dataset). 
}

\myitem{Model simplicity vs. accuracy.} As a final step, we investigate whether simpler models could be used to accurately capture the user satisfaction. Simpler models are more appealing since they require less data/features (practicality) and involve less terms (explainability). To this end, we build an OR model with only the $N$ ($N\leq 9$) features with the highest weights, calculate the MAE as before, and plot the results in Fig.~\ref{fig:MAE-vs-nb-features}. Our results show that \pavlos{(i) taking account only the most important feature ($\min\{QoS,Int\}$) is enough to improve the prediction of a Vanilla-RS by XX, (ii) including one more feature further reduces by XX, and (iii) considering the top 4 features gets already very close to the best achieved accuracy.}


% \begin{figure}
% \centering
% \subfigure[QoS vs. Int]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__QoS_vs_Int__SVR__rm_outliers_True.eps}\label{fig:2D-qos-int-SVR}}
% \hspace{0.05\linewidth}
% \subfigure[QoS vs. QoR]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__QoS_vs_QoR__SVR__rm_outliers_True.eps}\label{fig:2D-qos-qor-SVR}}
% %\subfigure[min\{QoS,Int\} vs. max\{QoS,Int\}]{\includegraphics[width=\mycustomwidth]{./figures/ML_plots/fig_class_boundaries_2D__min_QoS_Int_vs_max_QoS_Int__SVR__rm_outliers_True.eps}\label{fig:2D-qos-int-MLPR}}
% \caption{\pavlos{Probably this figure will not be a part of the paper} QoE predictions of a SVR (Support Vector Regression) model with parameters/features (a) QoS and Int, and (b) QoS and QoR%min\{QoS,Int\} and max\{QoS,Int\}
% . The axes correspond to the feature values (from 1 to 5 stars), the colored areas denote the QoE predictions (from 1 to 5 stars; dark blue corresponds to 1 and light green to 5), and the lines are the boundaries between the different QoE areas.}
% \label{fig:2D-SVR}
% \end{figure}



